Compositional Chain-of-Thought Prompting for Large Multimodal Models

The combination of strong visual backbones and Large Language Model (LLM) reasoning has led to Large Multimodal Models (LMMs) becoming the current standard for a wide range of vision and language (VL) tasks. However, recent research has shown that even the most advanced LMMs still struggle to capture aspects of compositional visual reasoning, such as attributes and relationships between objects. One solution is to utilize scene graphs (SGs)--a formalization of objects and their relations and attributes that has been extensively used as a bridge between the visual and textual domains. Yet, scene graph data requires scene graph annotations, which are expensive to collect and thus not easily scalable. Moreover, finetuning an LMM based on SG data can lead to catastrophic forgetting of the pretraining objective. To overcome this, inspired by chain-of-thought methods, we propose Compositional Chain-of-Thought (CCoT), a novel zero-shot Chain-of-Thought prompting method that utilizes SG representations in order to extract compositional knowledge from an LMM. Specifically, we first generate an SG using the LMM, and then use that SG in the prompt to produce a response. Through extensive experiments, we find that the proposed CCoT approach not only improves LMM performance on several vision and language VL compositional benchmarks but also improves the performance of several popular LMMs on general multimodal benchmarks, without the need for fine-tuning or annotated ground-truth SGs. Code: https://github.com/chancharikmitra/CCoT

==> sec/3_methods_old.tex <==
\section{Compositional Chain-of-Thought}
\label{sec:CCoT}


We begin by describing the standard LMM architecture (\Secref{sec:CCoT:preliminaries}). We then introduce our two-step chain-of-thought approach: first is scene graph generation (\Secref{sec:CCoT:sgg}) and second is response generation (\Secref{sec:CCoT:rg}). Our method is illustrated in~\figgref{fig:full_pipeline}. 


%{\smodel} is a novel multimodal zero-shot prompting method that leverages scene graph generation as an intermediate reasoning step. First, being a zero-shot method means that {\smodel} does not require scene-graph reasoning examples as compared to a few-shot methods []. This has the very important benefit of not requiring any ground truth scene graphs. Furthermore, the decision to use scene graphs is specifically tailored for LMMs. Visual questions are highly diverse, requiring both simple image understanding as well as reasoning about non-image concepts using visual details. Scene graphs address this variability as they apply to a very broad range of visual questions making our method highly generalizable. Additionally, the structured nature of scene graphs means that they can be generated using a very compact prompt, which is crucial as 
%most LMMs have smaller context lengths due to having both visual and textual features as input.
%Finally, it is especially important to note that our method relies only on a single LMM model, requiring no finetuning or helper LLM to reason over language information.


\subsection{Preliminaries}
\label{sec:CCoT:preliminaries}

LMMs are multimodal models that directly reason over both vision and language modalities. They are typically given inputs of one image $I$ and an associated task prompt in text form $P_{\mathrm{in}}$ (e.g., questions, caption generation, etc.). 
%In multimodal benchmarks, in particular, this prompt usually consists of a variety of objectives like a visual question or identification task.
Each modality is then encoded into a shared embedding space that a language model $f_{\theta}(\cdot)$ (parameterized by $\theta$) can reason over. More concretely, the image is encoded using a trainable vision encoder $v_{\phi}(\cdot)$ (parameterized by $\phi$), while the task prompt is tokenized and then encoded using a fixed language embedding $l$. Given an input image $I$ and input task prompt $P_\mathrm{in}$, the language model (typically an LLM) then outputs a text response $R$.

\begin{equation}
    R = f(v_\phi(I), l(P_\mathrm{in}))
\end{equation}

% This describes a single forward pass of an LMM. 
%Existing LMMs are trained via visual instruction tuning datasets that consist of images paired with complex visual reasoning tasks like question-answering, conversations, and detailed descriptions\cite{liu2023llava} like question-answering and detailed descriptions []. 
The exact LMM sub-modules of the LLM, vision encoding architecture, and pretraining method for parameters ${\theta, \phi}$ differ between models but the overarching method described above remains the same. 

We propose {\smodel}, a zero-shot chain-of-thought prompting method that leverages scene graph generation to improve an LMM's compositional visual understanding and multimodal reasoning.  Notably, this method does not require any finetuning as it is purely prompting-based. Furthermore, no annotated SGs are required as the method is zero-shot. Ultimately, our method is centered around a scene-graph generation prompt $S_\mathrm{in}$ that can be integrated into $P_\mathrm{in}$ such that the LMM can output a scene graph $S_\mathrm{g}$ as an intermediate multimodal reasoning step to output better responses to task prompt, such as questions, classification, or caption generation. 


\subsection{Part 1: Scene-Graph Generation}
\label{sec:CCoT:sgg}
%\input{figs/fig_3_ablations}
In addressing the challenge of LMMs viewing images as a ``bag of objects," a limitation highlighted in previous works \cite{Ma2022CREPE, winoground, herzig2023incorporating, doveh2022teaching}, our method introduces a novel approach to enhance compositional visual understanding. We generate a scene graph of an image as an intermediate chain of thought reasoning step, recognizing that complex visual reasoning often requires an understanding of not just objects but also their attributes and relationships. To solve this ``bag-of-objects'' problem, our first prompt instructs the LMM to systematically construct a scene graph with three key properties: the identification of relevant \textit{objects}, their \textit{attributes}, and the \textit{relationships} between them. This approach is grounded in the intuition that objects in an image are the atomic units through which humans reason.

The scene graph is designed to be relevant to the input image and text, and we further condition its format to be in JSON. This standardization in JSON format is intended to facilitate easier interpretation by the LMM. By systematically organizing visual information through the inclusion of objects, relationships, and attributes in the scene graphs, we enable more structured and comprehensive reasoning. The full prompt, showcasing this structured approach, is illustrated in Figure~\ref{fig:full_pipeline}.



This method represents a core novel contribution of our work, aiming to overcome the limitations of existing multimodal reasoning models and enhance the compositional understanding of LMMs.


Our first prompt to the LMM, which we denote as $P_\mathrm{in}^{(1)}$ is constructed by using the input image $I$, task prompt $P_\mathrm{in}$, and most notably the \textbf{scene-graph generation prompt} $S_\mathrm{in}$ (showed in red under Scene-Graph Generation in Figure~\ref{fig:full_pipeline}). The full prompt is as follows:
\begin{equation}
     P_\mathrm{in}^{(1)} = \text{``[$I$] [$P_\mathrm{in}$] [$S_\mathrm{in}$]"}
\end{equation} 
where $[\cdot]$ indicates slots for inserting the individual elements of the prompt. The LMM thus generates a scene graph as follows:

\begin{equation}
    S_\mathrm{g} = f(v_\phi(I), l(P_\mathrm{in}^{(1)}))
\end{equation}

%As all of the questions featured in our evaluations are in a question-answer format, the example presented in Figure~\ref{fig:full_pipeline} aligns with this. But even with a change in question format, the prompt only requires minor changes in the $S_\mathrm{i}$ sub-prompt. This prompt is fed to the LMM and a scene graph $S_\mathrm{g}$ is generated.

\subsection{Part 2: Response Generation}
\label{sec:CCoT:rg}
Now that the LMM has generated a scene graph $S_\mathrm{g}$ for the specific task prompt, we use it as part of its reasoning when generating a response. The LMM is provided with the original task prompt, image, and corresponding generated SG so that all three can be jointly used as context to respond to this new task prompt. The overall input prompt for response generation is thus given as follows:

\begin{equation}
    P_\mathrm{in}^{(2)} = \text{``[$I$] [$S_\mathrm{g}$] [$P_\mathrm{in}$] [$C$] [$E$]"}
\end{equation}
%\roei{what Ti0 and Ti1 are?} \roei{Actually Ti1 was already defined in (2)!}\roei{You need to fix the notations it's not clear what's going on.}\roei{consider replacing to: Ti:=Q, Ti1 :=[Ii,Ti,Si] (as you did), Ti2:=[Ii,Sg,Ti1,C,E]?}

%\roei{where Ii is the image, Sg is the predicted scene graph, and so on.}
In addition to the input image $I$, original task prompt $P_\mathrm{in}$, and generated scene graph $S_\mathrm{g}$, we insert a context sentence $C$ and an answer extraction sentence $E$. $C$ briefly instructs the LMM to use the provided context. Concretely, this is given by ``Use the image and scene graph as context and answer the following question:''. Finally, while the flexibility of LLM text generation is a great modeling choice for high-level multimodal reasoning, this flexibility also makes response generation in a specific format non-trivial. Many multimodal benchmarks are in a multiple-choice format, for example. Since we evaluate our method on these types of benchmarks, a short additional sub-prompt $E$ (usually a conditioning sentence) is required to return the answer as a letter. For example, our answer extraction sub-prompt ``Answer with the option's letter from the given choices directly" is taken from LLaVA-1.5~\cite{liu2023llava15} as it has been shown to be reliable on large multiple-choice benchmarks. However, this method can be easily generalized to other answer formats like short answers or detailed descriptions by modifying or completely removing $E$. Thus, the LMM generates a final response  $R$ to the original image, task prompt pair $(I, P_\mathrm{in})$ as follows:

\begin{equation}
    R = f(v_\phi(I), l(P_\mathrm{in}^{(2)}))
\end{equation}


%\roei{Why To2 has the number 2? Just refer to it as O the output. Ping me where you see it. We need to improve the notations.}

